DC3: A learning method for optimization with hard constraints

Large optimization problems with hard constraints arise in many settings, yet classical solvers are often prohibitively slow, motivating the use of deep networks as cheap "approximate solvers." Unfortunately, naive deep learning approaches typically cannot enforce the hard constraints of such problems, leading to infeasible solutions. In this work, we present Deep Constraint Completion and Correction (DC3), an algorithm to address this challenge. Specifically, this method enforces feasibility via a differentiable procedure, which implicitly completes partial solutions to satisfy equality constraints and unrolls gradient-based corrections to satisfy inequality constraints. We demonstrate the effectiveness of DC3 in both synthetic optimization tasks and the real-world setting of AC optimal power flow, where hard constraints encode the physics of the electrical grid. In both cases, DC3 achieves near-optimal objective values while preserving feasibility.

==> Constrained Optimization/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}

\iffalse
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\fi

\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}

\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Constrained Optimization/tables/acopf.tex <==
\begin{table}[t]
    \centering
  {\small  \begin{tabular}{lllllll}
\toprule
{} &   Obj. value &      Max eq. &     Mean eq. &    Max ineq. &   Mean ineq. &            Time (s) \\
\midrule
Optimizer                &  3.81 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  \red{0.949 (0.002)} \\
DC3                        &  \blue{3.82 (0.00)} &  \blue{0.00 (0.00)} &  \blue{0.00 (0.00)} &  \blue{0.00 (0.00)} &  \blue{0.00 (0.00)} &     \blue{0.089 (0.000)} \\
DC3, $\neq$                &  3.67 (0.01) &  \red{0.14 (0.01)} &  \red{0.02 (0.00)} &  0.00 (0.00) &  0.00 (0.00) &    0.040 (0.000) \\
DC3, $\not\leq$ train      &  3.82 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  0.00 (0.00) &     0.089 (0.000) \\
DC3, $\not\leq$ train/test &  3.82 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  \red{0.01 (0.00)} &  0.00 (0.00) &     0.039 (0.000) \\
DC3, no soft loss          &  3.11 (0.05) &  \red{2.60 (0.35)} &  \red{0.07 (0.00)} &  \red{2.33 (0.33)} &  \red{0.03 (0.01)} &    0.088 (0.000) \\
NN                         &  3.69 (0.02) &  \red{0.19 (0.01)} &  \red{0.03 (0.00)} &  0.00 (0.00) &  0.00 (0.00) &     0.001 (0.000) \\
NN, $\leq$ test            &  3.69 (0.02) &  \red{0.16 (0.00)} &  \red{0.02 (0.00)} &  0.00 (0.00) &  0.00 (0.00) &     0.040 (0.000) \\
Eq.~NN                    &  3.81 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  \red{0.15 (0.01)} &  0.00 (0.00) &     0.039 (0.000) \\
Eq.~NN, $\leq$ test       &  3.81 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  \red{0.15 (0.01)} &  0.00 (0.00) &     0.078 (0.000) \\
\bottomrule
\end{tabular}}
    \caption{Results on ACOPF over 100 test instances. We compare the performance of DC3 and other algorithms according to the metrics described in Table \ref{tab:simple-50-50}. We find again that baseline methods violate feasibility (as shown in \red{red}), while DC3 gives a feasible and near-optimal output about $10\times$ faster than the \texttt{PYPOWER} optimizer, even assuming that \texttt{PYPOWER} is fully parallelized.
\vspace{-0.1in}}
    \label{tab:acopf}
\end{table}

==> Constrained Optimization/tables/nonconvex.tex <==
\begin{table}[t]
    \centering
{\small \begin{tabular}{lllllll}
\toprule
{} &     Obj.~value & Max eq.& Mean eq.& Max ineq.& Mean ineq.&           Time (s) \\
\midrule
Optimizer                 &  -11.59 (0.00) &  0.00 (0.00) &   0.00 (0.00) &    0.00 (0.00) &     0.00 (0.00) &  \red{0.121 (0.000)} \\
DC3                        &  \blue{-10.66 (0.03)} &  \blue{0.00 (0.00)} &   \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &     \blue{0.00 (0.00)} &  \blue{0.013 (0.000)} \\
DC3, $\neq$                &  -10.04 (0.02) &  \red{0.35 (0.00)} &   \red{0.13 (0.00)} &    0.00 (0.00) &     0.00 (0.00) &  0.009 (0.000) \\
DC3, $\not\leq$ train      &   -0.29 (0.67) &  0.00 (0.00) &   0.00 (0.00) &    \red{0.01 (0.01)} &     0.00 (0.00) &  0.010 (0.004) \\
DC3, $\not\leq$ train/test &   -0.27 (0.67) &  0.00 (0.00) &   0.00 (0.00) &    \red{0.03 (0.03)} &     0.00 (0.00) &  0.001 (0.000) \\
DC3, no soft loss          &  -13.81 (0.00) &  0.00 (0.00) &   0.00 (0.00) &   \red{15.21 (0.04)} &     \red{2.33 (0.01)} &  0.013 (0.000) \\
NN                         &  -10.02 (0.01) &  \red{0.35 (0.00)} &   \red{0.13 (0.00)} &    0.00 (0.00) &     0.00 (0.00) &  0.001 (0.000) \\
NN, $\leq$ test            &  -10.02 (0.01) &  \red{0.35 (0.00)} &   \red{0.13 (0.00)} &    0.00 (0.00) &     0.00 (0.00) &  0.009 (0.000) \\
Eq.~NN                     &   -3.88 (0.56) &  0.00 (0.00) &   0.00 (0.00) &    \red{6.87 (0.43)} &     \red{0.72 (0.05)} &  0.001 (0.000) \\
Eq.~NN, $\leq$ test        &  -10.99 (0.03) &  0.00 (0.00) &   0.00 (0.00) &    \red{0.87 (0.04)} &     \red{0.06 (0.00)} &  0.013 (0.000) \\
\bottomrule
\end{tabular}}

    \caption{Results on our simple nonconvex task for 100 variables, 50 equality constraints, and 50 inequality constraints, with details as in Table \ref{tab:simple-50-50}. Since this problem is nonconvex, we use \texttt{IPOPT} as the classical optimizer. DC3 is differentiable and about $9\times$ faster than \texttt{IPOPT}, giving a near-optimal objective value and constraint satisfaction, in contrast to baseline deep learning-based methods which result in significant constraint violations.
\vspace{-0.1in}}
    \label{tab:nonconvex}
\end{table}

==> Constrained Optimization/tables/pseudocode.tex <==
{\small \begin{algorithm}[t!]
		\caption{Deep Constraint Completion and Correction (DC3)}
		\begin{algorithmic}[1]
		    \State \textbf{assume} equality completion procedure $\vp_x:\, \R^m\to \R^{n-m}$ \;\emph{// to solve equality constraints}
		    \State
		    \vspace{-0.05in}
		    \Procedure{train}{$X$}
		    \State \textbf{init} neural network $N_\theta : \mathbb{R}^d \to \mathbb{R}^m$
		    \While {not converged} for $x\in X$
		    \State \textbf{compute} partial set of variables $z = N_\theta(x)$
		    \State \textbf{complete} to full set of variables $\tilde{y} = \begin{bmatrix} z^T & \vp_x(z)^T \end{bmatrix}^T\in \R^n$
		    \State \textbf{correct} to feasible (or approx.~feasible) solution $\hat{y} = \rho^{(t_{\text{train}})}_x(\tilde{y})$
		    \State \textbf{compute} constraint-regularized loss $\ell_{\text{soft}}(\hat{y})$
		    \State \textbf{update} $\theta$ using  $\nabla_\theta \ell_{\text{soft}}(\hat{y})$
		    \EndWhile
		    \EndProcedure
		    \State
		    \vspace{-0.05in}
		    \Procedure{test}{$x$, $N_\theta$}
		    \State \textbf{compute} partial set of variables $z = N_\theta(x)$
		    \State \textbf{complete} to full set of variables $\tilde{y} = \begin{bmatrix} z^T & \vp_x(z)^T \end{bmatrix}^T$
		    \State \textbf{correct} to feasible solution $\hat{y} = \rho^{(t_{\text{test}})}(\tilde{y})$
		    \State \textbf{return} $\hat{y}$
		    \EndProcedure
		\end{algorithmic}
		\label{fig:pseudocode}
	\end{algorithm}
	}

==> Constrained Optimization/tables/simple-varyEq.tex <==
\begin{table}[t]
    \centering
 {\small   \begin{tabular}{lllllll}
\toprule
\multirow{3}{*}{\shortstack{Optimizers\\(OSQP, qpth)}} &Obj.~val. &   -27.26 (0.00) &  -23.13 (0.00) &  -15.05 (0.00) &  -14.80 (0.00) &  -4.79 (0.00) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\\hline
\multirow{3}{*}{DC3} & Obj.~val. &  \blue{-25.79 (0.02)} &  \blue{-20.29 (0.20)} &  \blue{-13.46 (0.01)} &  \blue{-13.73 (0.02)} &  \blue{-4.76 (0.00)} \\
                     & Max eq. &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &   \blue{0.00 (0.00)} \\
                     & Max ineq. &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &   \blue{0.00 (0.00)} \\\hline
\multirow{3}{*}{DC3, $\neq$} & Obj.~val. &  -22.59 (0.18) &  -20.40 (0.03) &  -12.58 (0.04) &  -13.36 (0.02) &  -5.27 (0.00) \\
                     & Max eq. &    \red{0.12 (0.01)} &    \red{0.24 (0.00)} &    \red{0.35 (0.00)} &    \red{0.47 (0.00)} &   \red{0.59 (0.00)} \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\\hline
\multirow{3}{*}{DC3, $\not\leq$ train} & Obj.~val. &  -25.75 (0.04) &  -20.14 (0.15) &   -1.39 (0.97) &  -13.71 (0.04) &  -4.75 (0.00) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    \red{0.02 (0.02)} &    0.00 (0.00) &   0.00 (0.00) \\\hline
\multirow{3}{*}{DC3, $\not\leq$ train/test} & Obj.~val. &  -25.75 (0.04) &  -20.14 (0.15) &   -1.23 (1.21) &  -13.71 (0.04) &  -4.75 (0.00) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    \red{0.09 (0.13)} &    0.00 (0.00) &   0.00 (0.00) \\\hline
\multirow{3}{*}{DC3, no soft loss} & Obj.~val. &  -66.79 (0.01) &  -40.63 (0.02) &  -21.84 (0.00) &  -15.56 (0.02) &  -4.76 (0.01) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\
                     & Max ineq. &  \red{122.52 (0.22)} &   \red{50.25 (0.14)} &   \red{23.83 (0.11)} &    \red{5.85 (0.18)} &   0.00 (0.00) \\\hline
\multirow{3}{*}{NN} & Obj.~val. &  -22.65 (0.12) &  -20.43 (0.03) &  -12.57 (0.01) &  -13.35 (0.03) &  -5.29 (0.02) \\
                     & Max eq. &    \red{0.11 (0.01)} &    \red{0.24 (0.00)} &    \red{0.35 (0.00)} &    \red{0.47 (0.00)} &   \red{0.59 (0.00)} \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\\hline
\multirow{3}{*}{NN, $\leq$ test} & Obj.~val. &  -22.65 (0.12) &  -20.43 (0.03) &  -12.57 (0.01) &  -13.35 (0.03) &  -5.29 (0.02) \\
                     & Max eq. &    \red{0.11 (0.01)} &    \red{0.24 (0.00)} &    \red{0.35 (0.00)} &    \red{0.47 (0.00)} &   \red{0.59 (0.00)} \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\\hline
\multirow{3}{*}{Eq.~NN} & Obj.~val. &  -27.20 (0.02) &  -22.74 (0.14) &   -9.16 (0.75) &  -14.64 (0.01) &  -4.74 (0.01) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\
                     & Max ineq. &    \red{0.43 (0.02)} &    \red{1.37 (0.09)} &    \red{8.83 (0.72)} &    \red{0.86 (0.05)} &   0.00 (0.00) \\\hline
\multirow{3}{*}{Eq.~NN, $\leq$ test} & Obj.~val. &  -27.20 (0.02) &  -22.76 (0.13) &  -14.68 (0.05) &  -14.65 (0.01) &  -4.74 (0.01) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &   0.00 (0.00) \\
                     & Max ineq. &    \red{0.42 (0.02)} &    \red{1.27 (0.09)} &    \red{0.89 (0.05)} &    \red{0.85 (0.05)} &   0.00 (0.00) \\
\bottomrule
\end{tabular} }
    \caption{Results on QP task for 100 variables and 50 inequality constraints, as the number of equality constraints varies as $10,30,50,70,90$. We compare the performance of DC3 and other algorithms according to objective value and maximum equality/inequality constraint violations averaged across test instances. (Standard deviations across 5 runs are shown in parentheses.) We find that neural network baselines give significantly inferior performance (shown in \red{red}) across all problems.}
    \label{tab:simple-vary-eq}
\end{table}

==> Constrained Optimization/tables/simple-varyIneq.tex <==
\begin{table}[h]
 {\small   \begin{tabular}{lllllll}
\toprule
                     &           &            10 &            30 &            50 &            70 &            90 \\
\midrule
\multirow{3}{*}{\shortstack{Optimizers\\(OSQP, qpth)}} & Obj.~val. &  -17.33 (0.00) &  -16.33 (0.00) &  -15.05 (0.00) &  -14.61 (0.00) &  -14.26 (0.00) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\\hline
\multirow{3}{*}{DC3} & Obj.~val. &  \blue{-15.18 (0.31)} &  \blue{-13.90 (0.20)} &  \blue{-13.46 (0.01)} &  \blue{-10.52 (0.93)} &  \blue{-11.77 (0.07)} \\
                     & Max eq. &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} \\
                     & Max ineq. &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} &    \blue{0.00 (0.00)} \\\hline
\multirow{3}{*}{DC3, $\neq$} & Obj.~val. &  -15.66 (0.05) &  -14.10 (0.04) &  -12.58 (0.04) &  -12.10 (0.03) &  -11.72 (0.03) \\
                     & Max eq. &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\\hline
\multirow{3}{*}{DC3, $\not\leq$ train} & Obj.~val. &  -15.60 (0.30) &  -13.83 (0.15) &   -1.39 (0.97) &  -11.14 (0.05) &  -11.76 (0.06) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    \red{0.02 (0.02)} &    0.00 (0.00) &    0.00 (0.00) \\\hline
\multirow{3}{*}{DC3, $\not\leq$ train/test} & Obj.~val. &  -15.60 (0.30) &  -13.83 (0.15) &   -1.23 (1.21) &  -11.14 (0.05) &  -11.76 (0.06) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    \red{0.09 (0.13)} &    0.00 (0.00) &    0.00 (0.00) \\\hline
\multirow{3}{*}{DC3, no soft loss} & Obj.~val. &  -21.78 (0.01) &  -21.72 (0.03) &  -21.84 (0.00) &  -21.82 (0.01) &  -21.83 (0.00) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\
                     & Max ineq. &   \red{23.85 (0.52)} &   \red{23.54 (0.23)} &   \red{23.83 (0.11)} &   \red{23.73 (0.09)} &   \red{23.69 (0.06)} \\\hline
\multirow{3}{*}{NN} & Obj.~val. &  -15.66 (0.03) &  -14.10 (0.05) &  -12.57 (0.01) &  -12.12 (0.03) &  -11.70 (0.02) \\
                     & Max eq. &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\\hline
\multirow{3}{*}{NN, $\leq$ test} & Obj.~val. &  -15.66 (0.03) &  -14.10 (0.05) &  -12.57 (0.01) &  -12.12 (0.03) &  -11.70 (0.02) \\
                     & Max eq. &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} &    \red{0.35 (0.00)} \\
                     & Max ineq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\\hline
\multirow{3}{*}{Eq.~NN} & Obj.~val. &  -17.07 (0.20) &  -15.45 (0.09) &   -9.16 (0.75) &  -14.20 (0.06) &  -14.10 (0.10) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\
                     & Max ineq. &    \red{1.65 (0.22)} &    \red{1.79 (0.10)} &    \red{8.83 (0.72)} &    \red{2.26 (0.04)} &    \red{1.28 (0.05)} \\\hline
\multirow{3}{*}{Eq.~NN, $\leq$ test} & Obj.~val. &  -17.06 (0.20) &  -15.65 (0.09) &  -14.68 (0.05) &  -14.31 (0.06) &  -14.10 (0.10) \\
                     & Max eq. &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) &    0.00 (0.00) \\
                     & Max ineq. &    \red{1.53 (0.19)} &    \red{1.58 (0.08)} &    \red{0.89 (0.05)} &    \red{1.92 (0.04)} &    \red{1.25 (0.04)} \\
\bottomrule
\end{tabular}
 }
    \caption{Results on QP task for 100 variables and 50 equality constraints. The number of \emph{inequality} constraints varies as $10,30,50,70,90$. Content and interpretation as in Table \ref{tab:simple-vary-eq}.}
    \label{tab:simple-vary-ineq}
\end{table}

==> Constrained Optimization/tables/simple5050.tex <==
\begin{table}[t]
    \centering
{\small \begin{tabular}{lllllll}
\toprule
{} &     Obj.~value & Max eq. & Mean eq. & Max ineq. & Mean ineq. & Time (s) \\
\midrule
Optimizer (OSQP)                       &  -15.05 (0.00) &  0.00 (0.00) & 0.00 (0.00) &   0.00 (0.00) & 0.00 (0.00) &  0.002 (0.000) \\
Optimizer (qpth)                       &  -15.05 (0.00) &  0.00 (0.00) &  0.00 (0.00) &   0.00 (0.00) &  0.00 (0.00) &  \red{1.335 (0.012)} \\
DC3                                    &  \blue{-13.46 (0.01)} &  \blue{0.00 (0.00)} &  \blue{0.00 (0.00)} &   \blue{0.00 (0.00)} &  \blue{0.00 (0.00)} &  \blue{0.017 (0.001)} \\
DC3, $\neq$                      &  -12.58 (0.04) &  \red{0.35 (0.00)} &  \red{0.13 (0.00)} &   0.00 (0.00) &  0.00 (0.00) &  0.008 (0.000) \\
DC3, $\not\leq$ train          &   -1.39 (0.97) &  0.00 (0.00) &  0.00 (0.00) &   \red{0.02 (0.02)} &  0.00 (0.00) &  0.017 (0.000) \\
DC3, $\not\leq$ train/test &   -1.23 (1.21) &  0.00 (0.00) &  0.00 (0.00) &   \red{0.09 (0.13)} &  \red{0.01 (0.01)} &  0.001 (0.000) \\
DC3, no soft loss                      &  -21.84 (0.00) &  0.00 (0.00) &  0.00 (0.00) &  \red{23.83 (0.11)} &  \red{4.04 (0.01)} &  0.017 (0.000) \\
NN                                     &  -12.57 (0.01) &  \red{0.35 (0.00)} &  \red{0.13 (0.00)} &   0.00 (0.00) &  0.00 (0.00) &  0.001 (0.000) \\
NN, $\leq$ test            &  -12.57 (0.01) &  \red{0.35 (0.00)} &  \red{0.13 (0.00)} &   0.00 (0.00) &  0.00 (0.00) &  0.008 (0.000) \\
Eq.~NN                          &   -9.16 (0.75) &  0.00 (0.00) &  0.00 (0.00) &   \red{8.83 (0.72)} &  \red{0.91 (0.09)} &  0.001 (0.000) \\
Eq.~NN, $\leq$ test &  -14.68 (0.05) &  0.00 (0.00) &  0.00 (0.00) &   \red{0.89 (0.05)} &  \red{0.07 (0.01)} &  0.018 (0.001) \\
\bottomrule 
\end{tabular}}

    \caption{Results on QP task for 100 variables, 50 equality constraints, and 50 inequality constraints. We compare the performance of DC3 and other algorithms according to the objective value and max/mean values of equality/inequality constraint violations, each averaged across test instances. We also compare the total time required to run on all 833 test instances, assuming full parallelization. (Std.~deviations across 5 runs are shown in parentheses for all figures reported.) Lower values are better for all metrics. We find that methods other than DC3 and Optimizer violate feasibility (as shown in \red{red}). DC3 gives a feasible output with reasonable objective value $78\times$ faster than \texttt{qpth} and only $9\times$ slower than \texttt{OSQP}, which is optimized for convex QPs.}
    \label{tab:simple-50-50}
\end{table}

